Robust Dataset Distillation by Matching Adversarial Trajectories

Dataset distillation synthesizes compact datasets that enable models to achieve performance comparable to training on the original large-scale datasets. However, existing distillation methods overlook the robustness of the model, resulting in models that are vulnerable to adversarial attacks when trained on distilled data. To address this limitation, we introduce the task of ``robust dataset distillation", a novel paradigm that embeds adversarial robustness into the synthetic datasets during the distillation process. We propose Matching Adversarial Trajectories (MAT), a method that integrates adversarial training into trajectory-based dataset distillation. MAT incorporates adversarial samples during trajectory generation to obtain robust training trajectories, which are then used to guide the distillation process. As experimentally demonstrated, even through natural training on our distilled dataset, models can achieve enhanced adversarial robustness while maintaining competitive accuracy compared to existing distillation methods. Our work highlights robust dataset distillation as a new and important research direction and provides a strong baseline for future research to bridge the gap between efficient training and adversarial robustness.

==> sec/0_abstract.tex <==
\begin{abstract}
Dataset distillation aims to generate a compact dataset guided by a large-scale dataset, enabling models trained on the distilled dataset to achieve performance comparable to those trained on the original dataset. However, existing dataset distillation methods do not account for model robustness, making models trained on distilled data are vulnerable to adversarial attacks. To address this problem, we first propose the task of ``robust dataset distillation'', which aims to embed robustness to synthetic datasets along with the distillation process to solve the problem of poor robustness of models trained on distilled data. We propose an adversarial trajectory matching-based dataset distillation method named Matching Adversarial Trajectories (MAT) to solve this problem. Building upon trajectory-matching-based approaches, our method incorporates adversarial training into the trajectory generation process. Specifically, we include adversarial samples in the generation of training trajectories to obtain robust training trajectories. Subsequently, we enhance the robustness of the distilled data by matching these robust trajectories. This method enables models to attain adversarial robustness while maintaining comparable accuracy to other dataset distillation methods through standard training on the distilled dataset. We compared our approach with several existing dataset distillation methods. The results demonstrate that our method enhances model robustness without compromising accuracy.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Nowadays, deep learning has achieved remarkable success across various domains \cite{he2016deep, huang2017densely, dosovitskiy2020image, hoefler2021sparsity}. However, the rapid expansion of both data volumes and model parameters has resulted in significantly longer training processes for neural network models. This increase in training duration poses challenges to the practical application of deep neural network technologies. 
To address this issue, dataset distillation techniques have garnered substantial attention from researchers \cite{wang2018dataset, cui2022dc, gou2021knowledge, nguyen2021dataset}. Dataset distillation generates a smaller, synthesized dataset guided by the original data, enabling more efficient model training while preserving performance. It can accelerate the training process and reduce computational resource requirements.


A variety of dataset distillation-based methods have been developed in recent years \cite{qin2024label, yu2025teddy, huang2024overcoming, deng2024exploiting}. However, although dataset distillation offers significant efficiency gains, its adversarial robustness has not received sufficient attention from researchers. Models trained on distilled datasets are highly susceptible to adversarial attacks, similar to those trained on the original datasets \cite{mkadry2017towards, goodfellow2014explaining, ilyas2019adversarial}. This means that small, imperceptible perturbations to input data can lead to drastically incorrect predictions by the model. To promote the widespread use of dataset distillation techniques, this is a pressing issue to address.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{sec/static/overview.pdf}
    \caption{Overview of robust dataset distillation. Adversarial examples are generated from the original data. Subsequently, these adversarial samples are utilized to distill a robust dataset. Models trained exclusively on this distilled dataset through standard (natural) training procedures inherently acquire adversarial robustness.}
    \label{fig:overview}
\end{figure}
% Table \ref{tab:origin} compares the performance of models trained on the original CIFAR-10 dataset and distilled data in terms of robustness.
% \begin{table}[ht] % 
%     \centering
%     \caption{\textcolor{red}{Change to graph}Accuracy(\%) comparison between original and distilled CIFAR-10 Datasets. We set IPC = 50 for distilled data and $\epsilon$ = 4/255 for the PGD~\cite{mkadry2017towards} attack.} 
%     {%
%     \begin{tabular}{c|cc}
%         \toprule
%          \multicolumn{1}{c|}{Method} & \multicolumn{1}{c}{Standard} & \multicolumn{1}{c}{Adversarial} \\
%          \midrule
%         Whole Dataset & 82.82 $\pm$ 0.34 & 1.98 $\pm$ 0.20 \\
%         MTT~\cite{cazenavette2022dataset} & 62.73 $\pm$ 1.13 & 1.99 $\pm$ 0.27 \\
%         MAT(Ours) & 60.96 $\pm$ 0.80  & 7.81 $\pm$ 1.07 \\
%         \bottomrule
%     \end{tabular}%
%     }
%     \label{tab:origin}
% \end{table}

% \begin{figure}[!t]
%     \centering
%     \begin{subfigure}[b]{0.49\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{sec/static/vis_intro_bar_ipc10.pdf}
%         \caption{IPC 10}
%         \label{fig:adv_10}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.49\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{sec/static/vis_intro_bar_ipc50.pdf}
%         \caption{IPC 50}
%         \label{fig:adv_50}
%     \end{subfigure}

%     \caption{Adversarial accuracy (\%) performance comparison of distilled CIFAR-10 generated by different dataset distillation methods without adversarial training. We set IPC (images per class) to 10 and 50 to performed the experiments separately. The attack is PGD-10 \cite{mkadry2017towards} with $\epsilon$ = 4/255. As a comparison, we also added the adversarial accuracy of model naturally trained on the full dataset. DD denotes normal Dataset Distillation, here we use the MTT~\cite{cazenavette2022dataset}. And DD with AT and MAT (our method) represent the direct use of the adversarial training trajectory and the smoothed adversarial training trajectory, respectively.}
%     \label{fig:r}
% \end{figure}

Researchers have proposed various defense mechanisms, with adversarial training emerging as the most effective strategy \cite{athalye2018obfuscated, uesato2018adversarial}. However, directly applying these methods on distilled datasets is inappropriate. This is because adversarial training involves generating adversarial examples during the training process. This approach has a significant drawback: generating adversarial samples requires multiple iterations during training, making the process extremely time-consuming. Moreover, dataset distillation aims to reduce data size to enhance training efficiency, whereas the iterative nature of adversarial training significantly increases computational costs. This conflict undermines the efficiency benefits that distillation techniques aim to provide. Therefore how to obtain robustness via distillation data is a new and challenging problem.


%因此解决蒸馏数据的鲁棒性是一个新的且具有挑战的问题
% we propose a method that embeds robustness acquired during adversarial training into a newly distilled dataset, as illustrated in Fig.~(\ref{fig:enter-label}).
We named this task robust dataset distillation. As the name suggests, based on dataset distillation, it requires incorporating robustness into the dataset during the process of distilling the data, allowing the model to learn adversarial robustness on the new dataset directly through natural training. Fig.~\ref{fig:overview} shows the overview of this task.

A straightforward way to solve this problem is to use a dataset distillation method based on trajectory matching with adversarial trajectories. Trajectory-matching methods for dataset distillation involve using model variations on distilled data to match variations in the original dataset. The set of weights learned by the model on the original dataset is referred to as a trajectory. During distillation, changes in the model's weights on the distilled data are used to match the changes in the trajectories. However, we found that replacing the trajectories with adversarial trajectories not only fails to make the distilled data robust, but even compromises its accuracy in the natural state. We believe that this is due to the difficulty in fitting the trajectory caused by the rapid change of model weights as a result of adversarial training. As an improvement, we smoothed the original adversarial training trajectory to reduce the difficulty of fitting. Specifically, we employ a trajectory-matching-based dataset distillation approach that aligns the training trajectories of models on the original data by replacing them with smoothed adversarial training trajectories. 
% As shown in Fig.~\ref{fig:r}, our method (MAT) significantly improves the robustness. 
To the best of our knowledge, our work is the first to present ``robust dataset distillation'' and make an effort to solve it.

We validate our algorithm across multiple datasets, demonstrating that our method can enhance the robustness of trained models while maintaining accuracy comparable to that of other distilled datasets. For example, compared to MTT \cite{cazenavette2022dataset}, our method improves robustness by 5.82\% with a 1.77\% decrease in accuracy when setting IPC = 50 on the CIFAR-10 dataset. In addition, we validate our method using several adversarial training approaches, including PGD-AT \cite{mkadry2017towards}, TRADES \cite{zhang2019theoretically}, and MART \cite{wang2019improving}, thereby demonstrating the generality of our algorithm.

In this work, we make the following key contributions:
\begin{itemize}
    \item We propose a new problem named robust dataset distillation for the first time, which focuses on the robustness of distilled datasets, aiming to embed robustness into the dataset along with the distillation process. 
    \item We found that since model weights change rapidly during adversarial training, this leads to the inability of dataset distillation methods based directly on adversarial trajectory matching to embed robust features into compressed datasets. We smoothed the training trajectory by adding the EMA mechanism to adversarial training to mitigate this situation.
    \item Building on smooth adversarial training trajectories, we propose the Matching Adversarial Trajectory (MAT) approach, which creates a distilled dataset with inherent adversarial robustness by matching these trajectories.
\end{itemize}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=1\linewidth]{sec/static/overview.pdf}
%     \caption{Overview of robust dataset distillation. Adversarial examples are generated from the original data. Subsequently, these adversarial samples are utilized to distill a robust dataset. Models trained exclusively on this distilled dataset through standard (natural) training procedures inherently acquire adversarial robustness.}
%     \label{fig:overview}
% \end{figure}
% We conduct extensive experiments on various benchmark datasets to demonstrate the effectiveness of MAT. The results affirm that our method not only preserves accuracy comparable to models trained on original datasets but also significantly enhances adversarial robustness, validating the practical applicability of our approach.
%-------------------------------------------------------------------------
% \subsection{Language}

% All manuscripts must be in English.

% \subsection{Dual submission}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section, must be no longer than eight pages in length.
% The references section will not be included in the page count, and there is no limit on the length of the references section.
% For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for \confName\ \confYear.}

% Overlength papers will simply not be reviewed.
% This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
% The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

% Reviewers:
% note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


% \subsection{Paper ID}
% Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% \subsection{Mathematics}

% Please number all of your sections and displayed equations as in these examples:
% \begin{equation}
%   E = m\cdot c^2
%   \label{eq:important}
% \end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}


==> sec/2_formatting.tex <==
\section{Related Work}
\label{sec:formatting}

% All text must be in a two-column format.
% The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
% Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
% The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
% The second and following pages should begin 1 inch (2.54 cm) from the top edge.
% On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
% for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
% page.

%-------------------------------------------------------------------------
\subsection{Dataset distillation}
Dataset distillation, also known as dataset compression, has garnered significant attention as a means of reducing the size of training datasets while preserving their informational content. Early approaches primarily focused on core set selection \cite{farahani2009facility, sener2017active, welling2009herding}, which involves selecting representative samples from the original dataset for retention. However, these methods often suffer from performance limitations and scalability issues when applied to large-scale image datasets. 

Gradient matching-based methods \cite{zhao2020dataset} optimize the synthetic dataset by minimizing the discrepancy between the gradients obtained from training models on the synthetic and original data. Zhao \textit{et al.} \cite{zhao2021dataset} further innovated on this approach by introducing differentiable Siamese augmentation within gradient matching, thereby enhancing the effectiveness of dataset distillation. Feature distribution matching-based methods \cite{zhao2023dataset} have been developed to significantly lower the computational costs associated with dataset distillation. Zhao \textit{et al.} \cite{zhao2023improved} further refined these methods to enhance their performance. Representative works in this category include CAFE \cite{wang2022cafe}, which matches features across various network layers, and DataDAM \cite{sajedi2023datadam}, which focuses on matching feature attention maps. 

Trajectory matching-based methods~\cite{cazenavette2022dataset} optimize the synthetic dataset by aligning the parameter update trajectories of models trained on the original and synthetic data. Building on this, Du \textit{et al.} \cite{du2023minimizing} reduced the error in the distilled dataset by minimizing the accumulated trajectory, while Liu \textit{et al.} \cite{liu2024dataset} proposed an automated approach to match the closest synthetic data trajectories to the original data trajectories, improving the performance of the distilled data. 
These advancements collectively illustrate the progressive efforts in the field of dataset distillation to enhance efficiency, scalability, and performance. However, despite these advancements, no prior work has addressed adversarial robustness in distilled datasets, underscoring the significance of our approach in tackling this critical gap.



%-------------------------------------------------------------------------
\subsection{Adversarial defense}

Adversarial defenses aim to enhance model robustness against adversarial attacks. One of the most renowned training methods in this field is adversarial training \cite{mkadry2017towards, goodfellow2014explaining}, which involves generating adversarial examples during training and incorporating them into the learning process. Two classical instances of this approach are Fast Gradient Sign Method (FGSM) adversarial training \cite{goodfellow2014explaining}, which employs single-step gradient ascent, and Projected Gradient Descent (PGD) adversarial training \cite{mkadry2017towards}, which extends gradient-based attacks to multiple steps. In addition to these foundational methods, Zhang \textit{et al.} introduced TRADES \cite{zhang2019theoretically}, which investigates the trade-off between model accuracy and robustness. Wang \cite{wang2019improving} proposed an error classification-aware strategy to improve overall robustness. Furthermore, Wu \textit{et al.} \cite{wu2020adversarial} enhanced adversarial training by considering perturbations in the model's weights.  Besides, studies have shown that models pre-trained on large datasets exhibit stronger resistance to adversarial attacks \cite{hendrycks2019using}. Additionally, data augmentation \cite{rebuffi2021fixing} plays a significant role in enhancing robustness by generating diverse adversarial samples to enrich the training data.

\textcolor{red}{
Several other works have explored robust dataset distillation. For instance, Xue \textit{et al.}~\cite{xue2024towards} employs curvature regularization in the loss function to enhance the robustness of the dataset, while Wu \textit{et al.}~\cite{wu2022towards} utilize meta-learning to achieve a robust dataset. Unlike these approaches, our method starts by optimizing the training trajectories of the teacher model, embedding robustness into the learning process from the outset. In addition to this, the prior methods exhibit notable limitations: Wu \textit{et al.} produce a dataset comparable in size to the original, which reduces the efficiency gains of distillation, and Xue \textit{et al.} only evaluate under relatively weak adversarial attacks. In contrast, our work addresses both issues by generating a compact distilled dataset that not only cuts computational overhead but also maintains strong robustness under more demanding adversarial conditions.}

%-------------------------------------------------------------------------
% \subsection{Robust Dataset Distillation}

% For the benefit of author(s) and readers, please use the
% {\small\begin{verbatim}
%   \cref{...}
% \end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
% This will automatically insert the appropriate label alongside the cross-reference as in this example:
% \begin{quotation}
%   To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
%   It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
%   You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
% \end{quotation}
% If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
% {\small\begin{verbatim}
%   \Cref{...}
% \end{verbatim}}
% command. Here is an example:
% \begin{quotation}
%   \Cref{fig:onecol} is also quite important.
% \end{quotation}

% %-------------------------------------------------------------------------
% \subsection{References}

% List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
% When referenced in the text, enclose the citation number in square brackets, for
% example~\cite{Authors14}.
% Where appropriate, include page numbers and the name(s) of editors of referenced books.
% When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
% If you use the template as advised, this will be taken care of automatically.

% \begin{table}
%   \centering
%   \begin{tabular}{@{}lc@{}}
%     \toprule
%     Method & Frobnability \\
%     \midrule
%     Theirs & Frumpy \\
%     Yours & Frobbly \\
%     Ours & Makes one's heart Frob\\
%     \bottomrule
%   \end{tabular}
%   \caption{Results.   Ours is better.}
%   \label{tab:example}
% \end{table}

% %-------------------------------------------------------------------------
% \subsection{Illustrations, graphs, and photographs}

% All graphics should be centered.
% In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
% Instead use
% {\small\begin{verbatim}
%   \centering
% \end{verbatim}}
% at the beginning of your figure.
% Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
% Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
% Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
% You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

% When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
% {\small\begin{verbatim}
%    \usepackage{graphicx} ...
%    \includegraphics[width=0.8\linewidth]
%                    {myfile.pdf}
% \end{verbatim}
% }


% %-------------------------------------------------------------------------
% \subsection{Color}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

% If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
% Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Method}

Robust dataset distillation aims to create a smaller yet robust dataset \( \mathcal{S} \) from the original dataset \( \mathcal{D} \), enabling a model trained on \( \mathcal{S} \) to achieve performance comparable to that on \( \mathcal{D} \) while also gaining adversarial robustness without the need for inefficient adversarial training. In this section, we introduce our proposed method for dataset distillation, based on smooth robust trajectory matching. Building on previous work, we pre-train the model and preserve its training trajectories, which are subsequently matched multiple times. Instead of using standard training trajectories, we replace them with adversarial training trajectories.
\subsection{Preliminaries}
\textbf{Adversarial training.} Adversarial training is a classic and widely recognized method for enhancing model robustness against adversarial attacks. This approach involves generating adversarial examples by subjecting training samples to white-box attack techniques. The model is then trained on these adversarial examples, enabling it to learn and adapt, thereby improving its robustness. The process of adversarial training can be formalized as follows:
\begin{equation}\small
\min_{\theta} \mathbb{E}_{(x, y) \sim \mathcal{D}} \left[ \max_{\|x' - x\| \leq \epsilon} \mathcal{L}\left(f_{\theta}(x'), y\right) \right], 
\end{equation}
where \( x' \) denotes the adversarial example, \( \theta \) represents the model parameters, \( \mathcal{D} \) is the original dataset, \( (x, y) \) is an input sample and its corresponding label, \( \epsilon \) is the maximum allowed norm of the adversarial perturbation, \( \mathcal{L} \) is the loss function, \( f_{\theta} \) is the model function parameterized by \( \theta \), and \( y \) is the label.

From the formulation of adversarial training, we observe that it can be represented as a bi-level optimization problem. In each training iteration, it first requires gradient ascent to optimize the inner maximization problem, followed by gradient descent to optimize the outer minimization problem. This process is highly time-consuming when training.

\noindent\textbf{Robust Dataset.}  The purpose of a robust dataset is to incorporate adversarial robustness directly into the dataset. This approach allows the model to achieve robustness through gradient descent alone when trained on the dataset, significantly reducing computational costs. We formally express the optimization objective as follows:
\begin{equation}\small
\begin{aligned}
\min_{\mathcal{S} } \quad & \mathbb{E}_{(x, y) \sim \mathcal{D}_{\mathrm{Test}}} \left[ \max_{\|x' - x\| \leq \epsilon} \mathcal{L}\left(f_{\theta^{\mathcal{S}}}(x'), y\right) \right], \\
\text{s.t.} \quad & \theta^{\mathcal{S}} = \arg\min_{\theta} \mathcal{L}_{\mathcal{S}}(\theta),\label{eq:robust dataset}
\end{aligned}
\end{equation}
where $\mathcal{S}$ is the robust dataset, and $\theta^{\mathcal{S}}$ denotes the model parameters trained on $S$. 
This method aims to create a dataset that inherently contains adversarial robustness, enabling more efficient training while maintaining the model's ability to resist adversarial attacks. By embedding robustness into the data, we can simplify the training process and potentially achieve similar levels of adversarial resistance with reduced computational overhead.
\subsection{Matching Training Trajectories}
In the trajectory matching process, we follow previous work\cite{cazenavette2022dataset, du2023minimizing}. Similar to Eq. (\ref{eq:robust dataset}), the objective function for dataset distillation can be formalized as:
\begin{equation}\small
\begin{aligned}
\min_{\mathcal{S}} \quad & \mathcal{L}_{\mathcal{D}_{\mathrm{Test}}}\left(f(\theta^{\mathcal{S}})\right), \\
\text{s.t.} \quad & \theta^{\mathcal{S}} = \arg\min_{\theta} \mathcal{L}_{\mathcal{S}}(\theta),
\end{aligned}
\end{equation}
where $\mathcal{S}$ represents the distilled small dataset, $\mathcal{L}_{\mathcal{D}_{\mathrm{Test}}}$ is the loss function on the original test dataset, $\theta$ denotes the model parameters, and $f^{\mathcal{S}}_{\theta}$ denotes the model trained on the distilled dataset $\mathcal{S}$.

Dataset distillation based on trajectory matching first requires selecting a model and training it on the complete original dataset. During training, we save the model parameters at the end of each epoch. These sequential model weights recorded over epochs form a trajectory that guides the distillation process.

More specifically, in each iteration during distillation training, we randomly select a timestamp $t$ that is smaller than the preset maximum timestamp $T$ and pick the corresponding model weight $\theta^{\mathcal{D}}_t$ at this time point as the start weight. The weight parameter of the trajectory at timestamp $t+M$, \textit{i.e.}, $\theta^\mathcal{D}_{t+M}$, serves as the target weight. Meanwhile, the student model is trained on the distilled dataset through $N$ gradient descent steps to obtain $\theta^\mathcal{S}_{t+N}$. After training the student model, we optimize the matching of the student model's parameters $\theta^\mathcal{S}_{t+N}$ to the target parameters $\theta^\mathcal{D}_{t+M}$. The discrepancy between the student and teacher trajectories is defined by the difference in model weights, normalized by the weight change magnitude $\Delta \theta = \|\theta^\mathcal{D}_{t+M} - \theta^\mathcal{D}_t\|$. The objective of the matching process can be formulated as:
\begin{equation}\small
L_{\text{match}} = \frac{\|\theta^\mathcal{S}_{t+N} - \theta^\mathcal{D}_{t+M}\|^2}{\|\theta^\mathcal{D}_{t+M} - \theta^\mathcal{D}_{t}\|^2}.
\end{equation}
The overall goal of trajectory matching is to minimize the aforementioned objective function, ensuring that the student model’s parameters closely track the changes in the teacher’s trajectory. By doing so, the distilled dataset is optimized to capture the training dynamics of the full dataset, thereby enhancing the student model's performance on the distilled data. In addition, based on the original method, ATT~\cite{liu2024dataset} proposes a strategy for automatically selecting the optimal parameter $N$ as shown below: 
\begin{equation}\small
N = \arg\min_{N} \|\theta^\mathcal{S}_{t+N} - \theta^\mathcal{D}_{t+M}\|^2.
\end{equation}
This formula means that the student model weights closest to the target weights will be selected during trajectory matching, avoiding the errors associated with artificially setting fixed parameters. Our methodology also references this approach.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{sec/static/method.pdf}
%     \caption{Workflow of trajectory generation in our method. Unlike previous approaches illustrated on the left, which preserve trajectories through standard (natural) training, our method enhances model robustness via adversarial training and applies EMA to smooth the model's training trajectories.}
%     \label{fig:method}
% \end{figure}

\subsection{Generating Adversarial Buffer}
To achieve a robust dataset, an intuitive approach is to replace the original training process with adversarial training. Adversarial training introduces adversarial examples during training to improve the model’s robustness against input perturbations. Specifically, by using the adversarially robust training trajectory as a guide, the training trajectory of the distilled dataset can be aligned with that of adversarial training. The goal is to enable the model to achieve adversarial robustness through natural training on the distilled dataset alone. However, our experiments revealed that this approach did not improve the robustness of the distilled data as expected. On the contrary, it significantly reduced the model's accuracy.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{sec/static/method.pdf}
    \caption{Workflow of trajectory generation in our method. Unlike previous approaches illustrated on the left, which preserve trajectories through standard (natural) training, our method enhances model robustness via adversarial training and applies EMA to smooth the model's training trajectories.}
    \label{fig:method}
\end{figure}

To investigate this issue further, we analyzed the cause and concluded that the rapid changes in model weights during adversarial training result in significant parameter discrepancies at various epochs along the trajectory. This drastic fluctuation in weights complicates the accurate matching of trajectories during the distillation process, leading to suboptimal performance. To verify this hypothesis, we conducted a visual analysis of weight changes in Fig.~\ref{fig:loss}. The results confirmed that adversarial training induces significant weight changing, validating our assumption.


Based on these findings, we propose smoothing the adversarial training trajectory to address rapid weight changes. To achieve this, we adopt the classical Exponential Moving Average (EMA) algorithm. The EMA algorithm reduces weight fluctuations by taking a weighted average of the weights from previous and current iterations, thereby smoothing the training trajectory. Specifically, the original training trajectory follows the update rule of adversarial training, as described in the Fig.~\ref{fig:method}.

After introducing EMA, our new update rule becomes:
\begin{equation} \small
\begin{aligned}
& \theta^{\text{EMA}}_t = \alpha \theta^{\text{EMA}}_{t-1} + (1 - \alpha) \theta_t, \\
\text{s.t.} \quad & \theta_{t} = \theta_{t-1} - \eta \nabla_{\theta} \mathcal{L}\left(\theta_{t-1}, x', y\right),
\end{aligned}
\end{equation}
where \( \alpha \) is the smoothing coefficient, and \( \theta^{\text{EMA}}_t \) represents the EMA-smoothed model weights. $\eta$ is the learning rate, \( \theta_t \) represents the model weights at iteration \( t \), \( \eta \) is the learning rate, \( \nabla \mathcal{L} \) denotes the gradient of the loss function with respect to the model parameters, \( x' \) is the adversarial example, and \( y \) is the label. 

Fig.~\ref{fig:loss} shows that introducing the EMA mechanism significantly reduces the rate of weight change and enables the natural trajectory to converge more closely to the adversarial trajectory in the later stages of training.
